Linguistically-driven Multi-task Pre-training for Low-resource Neural Machine Translation

In the present study, we propose novel sequence-to-sequence pre-training objectives for low-resource machine translation (NMT): Japanese-specific sequence to sequence (JASS) for language pairs involving Japanese as the source or target language, and English-specific sequence to sequence (ENSS) for language pairs involving English. JASS focuses on masking and reordering Japanese linguistic units known as bunsetsu, whereas ENSS is proposed based on phrase structure masking and reordering tasks. Experiments on ASPEC Japanese--English & Japanese--Chinese, Wikipedia Japanese--Chinese, News English--Korean corpora demonstrate that JASS and ENSS outperform MASS and other existing language-agnostic pre-training methods by up to +2.9 BLEU points for the Japanese--English tasks, up to +7.0 BLEU points for the Japanese--Chinese tasks and up to +1.3 BLEU points for English--Korean tasks. Empirical analysis, which focuses on the relationship between individual parts in JASS and ENSS, reveals the complementary nature of the subtasks of JASS and ENSS. Adequacy evaluation using LASER, human evaluation, and case studies reveals that our proposed methods significantly outperform pre-training methods without injected linguistic knowledge and they have a larger positive impact on the adequacy as compared to the fluency. We release codes here: https://github.com/Mao-KU/JASS/tree/master/linguistically-driven-pretraining.

==> backup.tex <==
\begin{table}[t]
\begin{center}
\arrayrulecolor{blue}
%\resizebox{0.8\textwidth}{!}{
\begin{tabular}{cc c c c c}

      \toprule
      \multirow{2}{*}{\#} &\multirow{2}{*}{Model} &\multicolumn{2}{c}{En-Ko}&\multicolumn{2}{c}{Ko-En}\\
      %\midrule
      & & 20k & 94k & 20k & 94k \\
      \midrule
      \multicolumn{4}{l}{\textit{Main baselines}}\\
      0 & w/o pre-training & 1.3 & 2.1 & 2.9 & 4.5\\
      0* & optimized transformer & 2.1 & 3.7 & 3.9 & 8.3 \\
      1 &MASS & 2.9 & 4.5 & 5.6 & 9.6 \\
      \midrule
      \multicolumn{4}{l}{\textit{Proposed methods}}\\
      2 & PMASS & 2.4 & 4.3 & 5.2 & 9.4 \\
      3 & HFSS & 3.1 & 4.8 & \textbf{7.7}$^\dag$ & 10.3$^\dag$ \\
      4 & ENSS (1 + 3) & \textbf{3.2} & \textbf{5.0}$^\dag$ & 6.8$^\dag$ & \textbf{10.9}$^\dag$ \\
      \midrule
      \multicolumn{4}{l}{\textit{Other combinations}}\\
       & 2 + 3 & 3.0 & 4.7 & 7.0$^\dag$ & 10.6$^\dag$ \\
      \bottomrule
\end{tabular}
%}
\caption{\REVISE{BLEU scores for simulated low-resource settings for English--Korean News translation using 20k and 94k parallel sentences for fine-tuning. Results better than MASS with statistical significance $p<0.05$ are marked in \dag.} }
\label{en-ko}
 \end{center}
\end{table}



\begin{table}[t]
\begin{center}
\arrayrulecolor{blue}
%\resizebox{0.9\textwidth}{!}{
\begin{tabular}{crrrrrr}

      \toprule
      Hyperparameters & Default & 3k & 10k & 20k & 50k & 94k \\
      \midrule
      BPE operations & 30k & 5k & 10k & 10k & 12k & 15k \\
      Encoder/decoder layers & 6 & 2 & 2 & 2 & 2 & 2 \\
      Attention heads & 16 & 2 & 2 & 2 & 2 & 2\\
      Embedding dimension & 1024 & 512 & 512 & 512 & 512 & 512 \\
      Feed forward dimension & 4096 & 512 & 1024 & 1024 & 2048 & 2048 \\
      Dropout & 0.3 & 0.3 & 0.3 & 0.3 & 0.3 & 0.3 \\
      Label smoothing & 0.1 & 0.6 & 0.5 & 0.5 & 0.5 & 0.4 \\
      Batch size & 4096 & 4096 & 4096 & 4096 & 4096 & 8192 \\
      \bottomrule
\end{tabular}
%}
\caption{\REVISE{Hyperparameters for optimized transformer. ``Default" denotes the setting of transformer-big. For English-Japanese, BPE operations for ``Vanilla transformer-big" is 40k.}} 
\label{hyperp}
 \end{center}
\end{table}




\begin{table}[t]
\begin{center}
%\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ccccccccc}

      \toprule
      \multirow{2}{*}{Model} &\multicolumn{4}{c}{Ja-En}&\multicolumn{4}{c}{En-Ja}\\
      %\midrule
      &  3k &  10k & 20k & 50k & 3k & 10k & 20k & 50k\\
      \midrule
      MASS &8.8&13.8&17.2&21.2&9.1&16.0&20.6&25.0\\
      ENSS &\textbf{11.2}$^\dag$&\textbf{16.7}$^\dag$&\textbf{19.0}$^\dag$&22.1$^\dag$&\textbf{11.7}$^\dag$&\textbf{18.7}$^\dag$&\textbf{22.5}$^\dag$&27.0$^\dag$\\
      \midrule
      BART (text infilling)  & 3.1  & 11.1 & 15.5 & 20.7 & 5.6  & 14.9 & 19.8 & 25.6$^\dag$ \\
      BART + ENSS & 10.7$^\dag$ & 15.8$^\dag$ & 18.9$^\dag$ & \textbf{22.4}$^\dag$ & 10.6$^\dag$ & 17.6$^\dag$ & 21.2$^\dag$ & \textbf{27.2}$^\dag$ \\
      \bottomrule
\end{tabular}
%}
\caption{\REVISE{BLEU scores compared with BART for simulated low/high-resource settings for Japanese--English ASPEC translation using from 3k to 50k parallel sentences for fine-tuning. Results better than MASS with statistical significance $p<0.05$ are marked in \dag.} }
\label{ja-en-bart}
 \end{center}
\end{table}



\begin{table}[t]
\begin{center}
%\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c c c c c c c c c }

      \toprule
     \multirow{2}{*}{Model} &\multicolumn{4}{c}{Ja-Zh}&\multicolumn{4}{c}{Zh-Ja}\\
      %\midrule
      &  3k &  10k & 20k & 50k & 3k & 10k & 20k & 50k \\
      \midrule
      MASS &15.7&20.3&22.4&24.7&19.4&25.9&29.4&32.9\\
      JASS&\textbf{17.1}$^\dag$&\textbf{22.2}$^\dag$&\textbf{23.2}$^\dag$&\textbf{25.2}$^\dag$&21.6$^\dag$&\textbf{27.5}$^\dag$&\textbf{30.4}$^\dag$&\textbf{33.6}$^\dag$\\
      \midrule
      BART (text infilling) & 13.5 & 19.0 & 21.3 & 24.4 & 20.3$^\dag$ & 25.8 & 29.1 & 33.0 \\
      BART + JASS & \textbf{17.1}$^\dag$ & 21.3$^\dag$ & 23.1$^\dag$ & 25.0 & \textbf{21.9}$^\dag$ & \textbf{27.5}$^\dag$ & \textbf{30.4}$^\dag$ & \textbf{33.6}$^\dag$ \\
      \bottomrule
\end{tabular}
%}
\caption{\REVISE{BLEU scores compared with BART for simulated low-resource settings for Japanese--Chinese ASPEC translation using 3k to 50k parallel sentences for fine-tuning. Results better than MASS with statistical significance $p<0.05$ are marked in \dag.}} 
\label{ja-zh-bart}
 \end{center}
\end{table}







\begin{table}[t]
\begin{center}
%\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c c c c c c c c c}

      \toprule
      \multirow{2}{*}{Model} &\multicolumn{4}{c}{Ja-Zh}&\multicolumn{4}{c}{Zh-Ja}\\
      %\midrule
      &  3k &  10k & 20k & 50k & 3k & 10k & 20k & 50k \\
      \midrule
      MASS & 7.7 &15.4&18.3&23.4&9.6&17.6&23.3&27.1\\
      JASS&\textbf{12.0}$^\dag$&\textbf{17.0}$^\dag$&\textbf{20.1}$^\dag$&\textbf{25.0}$^\dag$&\textbf{16.6}$^\dag$&21.2$^\dag$&\textbf{26.5}$^\dag$&29.2$^\dag$\\
      \midrule
      BART (text infilling) & 5.9  & 14.0 & 18.0 & 21.8 & 8.7  & 17.8 & 24.2$^\dag$ & 28.5$^\dag$ \\
      BART + JASS & 11.4$^\dag$ & 16.5$^\dag$ & 19.4$^\dag$ & 24.3$^\dag$ & 16.2$^\dag$ & \textbf{22.5}$^\dag$ & 26.2$^\dag$ & \textbf{30.0}$^\dag$ \\
      \bottomrule
\end{tabular}
%}
\caption{\REVISE{BLEU scores compared with BART for simulated low-resource settings for Japanese--Chinese Wikipedia translation using from 3k to 50k parallel sentences for fine-tuning. Results better than MASS with statistical significance $p<0.05$ are marked in \dag.} }
\label{ja-zh2-bart}
 \end{center}
\end{table}

